Saturation-Aware Model Predictive Energy Management for Droop-Controlled Islanded Microgrids

In this paper, we propose a minimax model predictive control (MPC)-based energy management system that is robust with respect to uncertainties in renewable infeed and load. The MPC formulation includes a model of low-level droop control with saturation at the power and energy limits of the units. Robust MPC-based energy management systems tend to under-utilize the renewable energy sources to guarantee safe operation. In order to mitigate this effect, we further consider droop control of renewable energy sources. For a microgrid with droop-controlled units, we show that enhancing droop feedback with saturation enlarges the space of feasible control actions. However, the resulting controller requires to solve a mixed-integer problem with additional variables and equations representing saturation. We derive a computationally tractable formulation for this problem. Furthermore, we investigate the performance gained by using droop with saturation, renewable droop and combination of both in a case study.

==> closedLoop-dataVariation-1.tex <==
\toprule
 & \cost & \resInfeedEnergy & \thermalInfeedEnergy & \numberOfThermalSwitchingActions\\
\midrule
\PrescientMpc & $0.225$ & $0.155$ & $0.0466$ & $12$\\
\MinimaxMpcResDroopOffDroopSatOff & $0.255$ & $0.149$ & $0.0490$ & $22$\\
\MinimaxMpcResDroopOffDroopSatOn & $0.253$ & $0.150$ & $0.0488$ & $14$\\
\MinimaxMpcResDroopOnDroopSatOff & $0.233$ & $0.154$ & $0.0472$ & $18$\\
\MinimaxMpcResDroopOnDroopSatOn & $0.224$ & $0.155$ & $0.0466$ & $10$\\
\bottomrule


==> closedOpenLoop-dataVariation-1.tex <==
\toprule
 & \predictedObjective & \predictedResInfeedEnergyScenario & \predictedThermalInfeedEnergyScenario\\
\midrule
\PrescientMpc & $0.121$ & $0.169$ & $0.0136$\\
\MinimaxMpcResDroopOffDroopSatOff & $0.188$ & $0.150$ & $0.0136$\\
\MinimaxMpcResDroopOffDroopSatOn & $0.188$ & $0.150$ & $0.0136$\\
\MinimaxMpcResDroopOnDroopSatOff & $0.144$ & $0.162$ & $0.0136$\\
\MinimaxMpcResDroopOnDroopSatOn & $0.121$ & $0.169$ & $0.0136$\\
\bottomrule

